A Deep Conditioning Treatment of Neural Networks

We study the role of depth in training randomly initialized overparameterized neural networks. We give a general result showing that depth improves trainability of neural networks by improving the conditioning of certain kernel matrices of the input data. This result holds for arbitrary non-linear activation functions under a certain normalization. We provide versions of the result that hold for training just the top layer of the neural network, as well as for training all layers, via the neural tangent kernel. As applications of these general results, we provide a generalization of the results of Das et al. (2019) showing that learnability of deep random neural networks with a large class of non-linear activations degrades exponentially with depth. We also show how benign overfitting can occur in deep neural networks via the results of Bartlett et al. (2019b). We also give experimental evidence that normalized versions of ReLU are a viable alternative to more complex operations like Batch Normalization in training deep neural networks.

==> alt_header.tex <==
%!TEX root = paper.tex
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{amsthm}

% \newtheorem{conjecture}{Conjecture}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}
%\newtheorem{model}{Model}
%\newtheorem{problem}{Problem}
% \newtheorem{problem}{Problem}
% \newtheorem{model}{Model}
% \newtheorem{remark}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}

\title{A Deep Conditioning Treatment of Neural Networks}

% Three or more authors with the same address:
% \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
%  \Name{Author Name2} \Email{an2@sample.com}\\
%  \Name{Author Name3} \Email{an3@sample.com}\\
%  \addr Address}

% Authors with different addresses:
\altauthor{%
 \Name{Naman Agarwal} \Email{namanagarwal@google.com}\\
 \addr Google AI, Princeton
 \AND
 \Name{Pranjal Awasthi} \Email{pranjalawasthi@google.com}\\
 \addr Google Research
 \AND
 \Name{Satyen Kale} \Email{satyenkale@google.com}\\
 \addr Google Research
}

==> convolution.tex <==
%!TEX root = paper.tex

\section{Convolution Analysis}
\label{app:convolution}

\nacomment{The notation in this section can be better. Please suggest}

In this section we analyse convolutional neural networks. Lets begin with a description of CNN. The description will be based on one dimensional convolution but we will try to keep it as general as possible so as to accomodate 2 dimensional convolution as well. Consider a $d$-dimensional input. For every coordinate in $i \in [d]$ we have an associated \textit{patch} $P_i \subseteq [d]$. We assume that all patches have qual size $\{|P_i| = P\}_{i=0}^{d-1}$.  Let $C_l$ be the number of channels at layer $l$ with $C_0 = 1$. The representation at layer $l$ for an input $x$, $\phi_l(x)$ is described by two indices $i,c$ with $i$ representing the index inside a channel (therefore $i \in [d]$) and $c$ represents the index over the channels $c \in [C_l]$. The equation is now given by 

\[ [\phi_{l+1}(x)]_{i,c} = \frac{1}{\sqrt{C_{l+1} \cdot P}}\sum_{c' \in C_{l+1}} \sigma\left(\sum_{j \in P_i} w_{lj} \cdot [\phi_{l}(x)]_{j,c'} \right)\]
We will consider the case when $\{c_l \rightarrow \infty \}_{l = 1}^{\infty}$ successively. 

\subsection{Norm Analysis}

\newcommand{\cnorms}[1]{n_{\phi}^{#1}}
\newcommand{\pnorms}[1]{n_P^{#1}}

We now define the following quantities which will be useful to the analysis. Let $\cnorms{l} \in [\reals^{+}]^d$ be the vector that represents the norm of a coordinate of the representation across the channels. Formally 

\[ [\cnorms{l}]_i := \sum_{c \in C_{l}} [\phi_l]^2_{i,c}.\]

Further define a similar quantity for the patches which represents the norm across an entire patch. 

\[ [\pnorms{l}]_i := \sum_{j \in P_i} [\cnorms{l}]_j.\]

The following equation now follow in the infinite channel limit which is easy to see

\begin{equation}
	[\cnorms{l+1}]_i = \frac{\hat{\sigma}_l([\pnorms{l}]_i)}{P} 
\end{equation}

The above implies the following 

\begin{equation}
	[\pnorms{l+1}]_i = \frac{\sum_{j \in P_i} \hat{\sigma}_l([\pnorms{l}]_j)}{P}
\end{equation}

The above equation sets up a simple graph flow setup - the local value passes through the norm transfer filter and then sets itself to the average of the values of its neighbours. Some easy to see claims that follow - 

\begin{itemize}
	\item Notice that the fixed
 point of this happens when eatch patch has norm exactly 1. 
 \item Furthermore owing to our previous analysis we see that if every patch has norm $[0.5, \infty]$ we can start getting an exponential decay - to see this consider a potential function $\psi(a) = |1 - a|$. From our previous analysis we know that 
	\[ \psi(\hat{\sigma}_l(a)) \leq (1 - \alpha_{\sigma}) \psi(a)\]
	Owing to the convexity of the potential function we can easiy get the following conclusion - 
	 \[ \psi([\pnorms{l+1}]_i) \leq (1 - \alpha_{\sigma}) \frac{ \sum_{j \in P_i} \psi([\pnorms{l}]_j)}{P}\]

	\item As a next step I dont like the per patch lower bound. We should be able to do a first phase analysis too - or not - lets see. 
\end{itemize}




==> discussion.tex <==
%!TEX root = paper.tex

Our main result on conditioning (\pref{thm:main-infinite-width-top-layer} and \pref{thm:main-infinite-width-ntk}) and their applications clearly demonstrate the joint benefit of using deeper networks with non-linear activations from an optimization and generalization perspective. 
% Our \pref{ass:separation} is standard and has been used in prior works on optimization of neural networks via stochastic gradient descent \citep{allen2018convergence, zou-gu, du-zhai-poczos-singh}. \pref{ass:non-singularity} is stronger but is easily satisfied by randomly initialized one layer networks with popular activations such as the ReLU. We establish this in \pref{thm:one-layer-conditioning-sgn}. 

Using our conditioning analysis we obtain in \pref{cor:train_all_layers} that when training all layers of a deep enough network via gradient descent, the iteration complexity is {\em independent} of $n$ and the initial separation $\delta$, thereby clearly demonstrating the benefit of depth. This is in contrast to prior works where the iteration complexity depends polynomially in the depth $L$ and $1/\delta$ \citep{allen2018convergence, zou-gu, du-zhai-poczos-singh}. 
% For the case of training all the layers with ReLU activations, our improved analysis implies that (see \pref{thm:top-layer-general}) the width requirement only has a {\em logarithmic} dependence in $1/\delta$, as opposed to polynomial in $1/\delta$ in prior works. 

Finally, note that all our theorems and their implications hold for the case of normalized activations as defined in \pref{eq:normalization}. As discussed earlier, the only somewhat non-standard part of the normalization is the requirement that the activation is centered so that its expectation on standard normal inputs is 0. This requirement is not simply a limitation of our analysis but is inherently necessary since when working with uncentered activations, a similar analysis to the one in this paper shows all pairwise dot products approach 1 (rather than 0) at an exponential rate. 

% Beyond this fact, we note that the commonly used {\em batch normalization} (BatchNorm) operation \citep{ioffe2015batch} makes it possible to assume that activations are centered without loss of generality. BatchNorm is an essential operation for efficient training of deep networks: in this operation the input $x$ to a given layer $k$ is processed to obtain $x'$ where $x' = (x - \mu_B)/\sigma_B$ and $\mu_B$ and $\sigma_B$ are the mean and the standard deviation of the inputs for given batch $B$ of examples. It is evident from the definition of BatchNorm that the output of the operation is invariant to translation of the activation by a fixed constant. Thus, without loss of generality we can assume that the activation is centered.
 % This has the effect that the resulting activations are normalized to zero mean and unit variance, similar to the use of normalized activation function $\sigma(\cdot)$ in our work. 
% In this light, our results can be viewed as providing a theoretical justification for the superior optimization performance of BatchNorm that has been observed in practice.

==> neurips_header.tex <==
%!TEX root = paper.tex
\usepackage{neurips_2020}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amsthm}

% \newtheorem{conjecture}{Conjecture}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
% \newtheorem{fact}{Fact}
% \newtheorem{assumption}{Assumption}
% %\newtheorem{model}{Model}
% %\newtheorem{problem}{Problem}
% \newtheorem{problem}{Problem}
% \newtheorem{model}{Model}
% \newtheorem{remark}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}

\title{A Deep Conditioning Treatment of Neural Networks}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  Naman Agarwal \\
  Google Research \\
  \texttt{namanagarwal@google.com} \\
  \And
  Pranjal Awasthi \\
  Google Research \\
  \texttt{pranjalawasthi@google.com} \\
  \And
  Satyen Kale \\
  Google Research \\
  \texttt{satyenkale@google.com}
}
